Group-Sparse Model Selection: Hardness and Relaxations

Group-based sparsity models are proven instrumental in linear regression problems for recovering signals from much fewer measurements than standard compressive sensing. The main promise of these models is the recovery of "interpretable" signals through the identification of their constituent groups. In this paper, we establish a combinatorial framework for group-model selection problems and highlight the underlying tractability issues. In particular, we show that the group-model selection problem is equivalent to the well-known NP-hard weighted maximum coverage problem (WMC). Leveraging a graph-based understanding of group models, we describe group structures which enable correct model selection in polynomial time via dynamic programming. Furthermore, group structures that lead to totally unimodular constraints have tractable discrete as well as convex relaxations. We also present a generalization of the group-model that allows for within group sparsity, which can be used to model hierarchical sparsity. Finally, we study the Pareto frontier of group-sparse approximations for two tractable models, among which the tree sparsity model, and illustrate selection and computation trade-offs between our framework and the existing convex relaxations.

==> hierarchical.tex <==
%!TEX root = GroupSparse-ISIT.tex
\section{Generalizations}

We can generalize \eqref{eq:WMC} by introducing a sparsity constraint $K$ and allowing to individually select variables within a group. The generalised integer problem then becomes
\begin{equation}
\label{eq:GWMC}
%\begin{array}{cl}
%\maximize\limits_{\omega \in \mathbb{B}^\ngroups,~y \in \mathbb{B}^\dim} & \sum_{i=1}^N y_i x_i^2 \\
%\text{subject~to} & \A^\mathfrak{G} \omega \geq y  \\
%& \sum_{i=1}^\dim y_i \leq K \\
%& \sum_{j=1}^\ngroups \omega_j \leq G \; .
%\end{array}
\max\limits_{\omega \in \mathbb{B}^\ngroups,~y \in \mathbb{B}^\dim} \left \{ \sum_{i=1}^N y_i x_i^2 : \A^\mathfrak{G} \omega \geq y, \sum_{i=1}^\dim y_i \leq K , \sum_{j=1}^\ngroups \omega_j \leq G \right \} \; .
\end{equation}

We can modify the dynamic programming algorithm of Prop.\ref{prop:DP1}, in order to solve \eqref{eq:GWMC} (see proof in the Appendix).
\begin{prop}
\label{prop:DP2}
Given a loopless pairwise overlapping groups structure $\mathfrak{G}$, there exists a polynomial time dynamic programming algorithm that solves \eqref{eq:GWMC}.
\end{prop}

The generalized model allows to deal with hierarchical structures, such as regular trees, frequently encountered in image processing (e.g. denoising using wavelet trees).
In such cases, we often require to find $K$-sparse approximations such that the selected variables form a rooted connected sub-tree of the original tree.
This type of constraint can be represented by a group structure, where for each node in the tree we define a group consisting of that node and all its ancestors. 
When a group is selected, we also require that all its elements are selected as well and impose a sparsity constraint $K$, but not a group constraint $G$.
For this type of structures, we are able to establish the same results as for the loopless pairwise overlapping groups structures. Due to space limitations we leave the proofs to a longer version of the paper.

\begin{prop}
\label{prop:DP2}
Given a hierarchical group structure $\mathfrak{G}$, there exists a polynomial time dynamic programming algorithm that solves \eqref{eq:GWMC}.
\end{prop}

By relaxing both the group budget and the sparsity budget in \eqref{eq:GWMC} into regularization terms, we obtain a binary linear program, which can be solved in polynomial time if the constraint matrix is TU. 
We already established TU for loopless pairwise overlapping groups. 
TU also holds for hierarchical groups.
\begin{prop}
Hierarchical group structures lead to to totally unimodular constraints.
\end{prop}
